Balance Maximization in Signed Networks via Edge Deletions

In signed networks, each edge is labeled as either positive or negative. The edge sign captures the polarity of a relationship. Balance of signed networks is a well-studied property in graph theory. In a balanced (sub)graph, the vertices can be partitioned into two subsets with negative edges present only across the partitions. Balanced portions of a graph have been shown to increase coherence among its members and lead to better performance. While existing works have focused primarily on finding the largest balanced subgraph inside a graph, we study the network design problem of maximizing balance of a target community (subgraph). In particular, given a budget $b$ and a community of interest within the signed network, we aim to make the community as close to being balanced as possible by deleting up to $b$ edges. Besides establishing NP-hardness, we also show that the problem is non-monotone and non-submodular. To overcome these computational challenges, we propose heuristics based on the spectral relation of balance with the Laplacian spectrum of the network. Since the spectral approach lacks approximation guarantees, we further design a greedy algorithm, and its randomized version, with provable bounds on the approximation quality. The bounds are derived by exploiting pseudo-submodularity of the balance maximization function. Empirical evaluation on eight real-world signed networks establishes that the proposed algorithms are effective, efficient, and scalable to graphs with millions of edges.

==> 2_previous_work.tex <==
%\newpage
%\section{Related Work}
%% Balance in Signed graphs
% Signed graphs, balance, existing work
\paragraph{Balance in Signed Graphs.}
Signed graphs have been studied in the literature for a long time since the pioneering work by Harary \cite{harary1953notion}, who was particularly interested in the notion of balance in such graphs. The concept of balance was however first introduced by Heider \cite{heider1946attitudes} in his psychological study of sentiments. Later, Cartwright and Harary \cite{cartwright1956structural} extended Heider's concept of balance to the signed graphs. Most earlier works focused on testing the balance property in signed graphs. Examples include the pseudo-boolean programming formulation by Hammer \cite{hammer1977pseudo}, the linear-time algorithm of Harary and Kabell \cite{harary_kabell1980simple}, the minimum number of sign changes approach by Akiyama et al. \cite{akiyama1981balancing}.

% Problem variations for balance in signed graphs
Subsequently, over the years, a lot of problem variations related to the balance in signed graphs have been studied. Poljak and Turz\'{i}k addressed the finding maximum weight balanced subgraph problem and showed that it is equivalent to finding max-cut in a graph with general weight function. Other problems include finding balanced subgraphs that maximizes the number of vertices \cite{figueiredo2014maximum,ordozgoiti2020finding} and with maximum number of edges by DasGupta et al. \cite{dasgupta2007algorithmic} in the context of biological networks. H\"{u}ffner et al. \cite{huffner2007optimal} gave an exact algorithm for finding such balanced subgraphs using the idea of graph separators. While the above papers mostly focused on finding the existing balanced subgraph, in this paper, we focus on the problem of maximizing balance by deleting a few edges in the graph.

% Spectral approach for the problem
Most of the earlier works in the signed graphs discussed before relied on the properties of balance theory. Hou et al. \cite{hou2003laplacian} introduced a spectral approach to this problem. In particular, Hou et al. showed that a connected signed graph is balanced if and only if the smallest eigenvalue of its corresponding Laplacian matrix is 0. In fact, Hou \cite{hou-ams:2005} extended this result to analyze the degree of \textit{unbalancedness} of a signed graph. Recently, Ordozgoiti et al. \cite{ordozgoiti2020finding} also used a similar approach for maximizing the balance in signed graphs by removing vertices. In this paper, we present a spectral theory based approach to maximize balance of a given subgraph by perturbing (deleting) a few edges. 

%% Network design problem
\paragraph{Network Design Problems.} Network design consists of problems that study the modification of networks to achieve or optimize desirable properties. These problems first initiated based on vertex upgradation to decrease the delays on adjacent edges~\cite{paik1995}.
Recently a series of work studied the problem of optimizing shortest path distances by reducing node or edge weights~\cite{meyerson2009,dilkina2011,lin2015,medya2018noticeable}. Another type of design problems aim to increase the centrality of a node or a set of nodes by adding a small set of edges~\cite{crescenzi2015,ishakian2012framework,medya2018group}. Modifications of k-cores that measure network resilience have been also studied recently \cite{Laishram2018,zhang2017finding,zhu2018k}. Besides the optimization problem related to these structural properties, boosting or containing diffusion processes in networks were also investigated under well-known diffusion models such as Linear Threshold \cite{Khalil2014} and Independent Cascade \cite{kimura2008minimizing,chaoji2012recommendations}. However, in this paper, we address a network design problem that differs from the described ones in terms of the objective function, i.e., maximizing balance in networks. 

==> background.tex <==
\section{ Background on Signed graphs}
We collect some facts about signed graphs and their Laplacians with reference to the ``balance'' property. The primary reference is the paper by Hou~\cite{hou-ams:2005}.


\subsection{Graph-theoretic background}
\begin{definition}[Signed graph]
A {\em signed graph}, $\Gamma = (G, \sigma)$ is a simple undirected graph $G = (V,E)$ and mapping $\sigma : E \rightarrow \{-1, +1\}$, called its {\em edge labelling}, that assigns a sign to each edge. 
\end{definition}

Given a signed graph $((V,E),\sigma)$ we will sometimes use the notation $E^+ = \{ e \in E : \sigma(e) = +1\}$, $E^- = \{ e \in E : \sigma(e) = -1\}$. Given a walk $W$ we say the sign of the walk is $\sgn(W) = \prod_{e \in W} \sigma(e)$. 

\begin{definition}[Balanced graph]
A signed graph $\Gamma = ((V,E),\sigma)$ is said to be balanced if there is a partition $(V_1, V_2)$ of $V$ such that for every $(u,v)\in E$ with $\sigma(u,v) = -1$, $u \in V_1$ iff $v \in V_2$. 
\end{definition}

Here's a small proposition I have not seen explicitly argued anywhere.
\begin{proposition}
If a balanced graph is connected then the partition that achieves balance is unique.
\end{proposition}
\begin{proof}
Let $(V_1, V_2)$ and $(V_1',V_2')$ be two balanced partitions of the signed graph. Assume without loss of generality that there are $u,v \in V_1'$ such that $u \in V_1$ and $v \in V_2$. The fact that $(V_1,V_2)$ is a balanced partition means that every path from $u$ to $v$ must have a negative sign. However the fact that $(V_1',V_2')$ is a balanced partition implies that every path from $u$ to $v$ should have a positive sign since it should either visit vertices only in $V_1'$ or should cross between the two partitions an even number of times. This gives a contradiction.
\end{proof}

\begin{proposition}
A signed graph is balanced iff the sign of every cycle is positive.
\end{proposition}
\begin{proof}
If a graph is balanced and $(V_1, V_2)$ is the partition that achieves balance then every cycle must cross the partition an even number of times, hence every cycle must be positive.

Now assume every cycle is positive. We prove balance algorithmically by trying to colour the graph with two colours. Pick any vertex and colour it blue. Now begin a BFS from this vertex. Every time a new vertex is discovered, if it is discovered via a positive signed edge, colour it the same colour as the vertex from which it was discovered, otherwise colour it with the opposite colour (i.e. red if the discovering vertex is blue). 

To show that this colouring gives us a balanced partition assume towards contradiction there is either (a) a positive edge between two vertices of opposite colour or (b) a negative edge between two vertices of the same colour. Since such edges cannot be tree edges of the BFS, we find a cycle by tracing the paths up to the least common ancestors in the BFS tree of the two endpoints of the offending edge. In both case the union of these two paths with the edge give us a negative cycle which is a contradiction.
\end{proof}

Note that some authors, e.g. Hou~\cite{hou-ams:2005}, Li and Li~\cite{li-tjm:2016}, define a signed graph to be balanced if all cycles are positive.

\begin{proposition}
\label{prp:subgraphs}
Every proper subgraph (obtained by removing one or more vertices) of a balanced graph is balanced.
\end{proposition}
This is easy to see since if vertices are removed the balance partition can be formed by taking the appropriate subsets of the two sides of the balance partition of the original graph. If only edges are removed then the balance constraints are only eased and so they remain satisfied.

Note that the converse of Proposition~\ref{prp:subgraphs} is not true. A simple counterexample is a complete graph on 3 vertices with a single negative edge and two positive edges. Each proper subgraph is balanced but the graph itself is not balanced. 

\subsection{Algebraic background}

Suppose we have an unsigned undirected graph $G=(V,E)$ with non-negative edge weights $w: E \to \RR_+$. Let its adjacency matrix be $A(G)$, i.e. $A(G)_{ij} = w_{ij}$ for each $(i,j) \in E$.  the matrix $\mathcal{L}(G) = D(G)-A(G)$ is called its Laplacian where $D(G)$ is a diagonal $|V|\times |V|$ matrix with $D_{ii} = d_i = \sum_{j: (i,j) \in E} w_{ij}$, the degree of vertex $i$. We define now the Laplacian of a signed graph. 
\begin{definition}
The Laplacian of a signed graph $\Gamma = (G=(V,E), \sigma)$, denoted $L(\Gamma)$ is a symmetric matrix $|V| \times |V|$ matrix with $L_{ii} = d_i$, and  $L_{ij} = -\sigma(i,j)$ if $(i,j) \in E$ and 0 otherwise for $i\ne j$. 
\end{definition}
\textbf{SR: Isn't this definition missing the diagonal elements?\\ Corrected. Remarks below were correct to begin with. AB.}


\noindent{\bf Remarks.}
\begin{enumerate}
\item Suppose $G^+ = (V, E^+)$ and $G^- = (V, E^-)$, then $L(\Gamma) = D(G^+) - A(G^+) + D(G^-) + A(G^-) = \mathcal{L}(G^+) + D(G^-) + A(G^-)$.
\item If $A^\sigma$ is the signed adjacency matrix of $A$, i.e., $A^\sigma_{ij} = \sigma(i,j)$ for all $(i,j) \in E$, then $L(\Gamma) = A^\sigma \circ \mathcal{L}(G)$ where $\mathcal{L}(G)$ is the unsigned Laplacian and $\circ$ denotes the Hadamard product.
\end{enumerate}

\begin{proposition}
\label{prp:lap-sd}
\begin{enumerate}
\item For any signed graph $\Gamma$, $L(\Gamma)$ is positive semidefinite.
\item $L(\Gamma)$ has eigenvalue 0 iff $\Gamma$ is balanced.
\end{enumerate}
\end{proposition}
\begin{proof}
Note that for any $\bm{x} \in \RR^{|V|}$, 
\begin{equation}
\label{eq:qform}
\bm{x}^T L(\Gamma) \bm{x} = \sum_{(i,j) \in E^+} (\bm{x}_i - \bm{x}_j)^2  + \sum_{(i,j) \in E^-} (\bm{x}_i + \bm{x}_j)^2.
\end{equation}
This can be easily verified by opening out the RHS. Clearly the RHS is non-negative for any $\bm{x} \in \RR^{|V|}$.

Now, assume that the graph is balanced. This means there is a partition $(V_1,V_2)$ of $V$ such that $\sigma(u,v) = -1$ iff $u \in V_1$ and $v \in V_2$. Consider the vector 
\[ \bm{x}_u = \left\{ \begin{array}{rr}
1, & u \in V_1\\
-1, & u \in V_2
\end{array}\right.\] 
Putting this back in \eqref{eq:qform} we see that the RHS is 0. Since $L(\Gamma)$ is positive semidefinite, this is the minimum value the quadratic form can achieve, hence it is an eigenvalue.

Now assume 0 is an eigenvalue of $L(\Gamma)$. Suppose that $\bm{x}$ is the eigenvector with eigenvalue 0. Clearly this means that each term on the RHS of \eqref{eq:qform} has to be 0 for $\bm{x}$. Consider any $u \in V$. For all neighbours $v$ of $u$ such that $\sigma(u,v) = 1$, we must have that $\bm{x}_v = \bm{x}_u$ and all $v$ such that $\sigma(u,v) = -1$ must have $\bm{x}_v = - \bm{x}_u$. Pick an arbitrary vertex $v_0$ and set $\bm{x}_{v_0} = 1$. This determines the values of all $\bm{x}_v$ such that $v$ is in the same connected component as $v_0$. Continue the process till all nodes are covered. The required partition is $V_1 =\{u: \bm{x}_u = 1\}$ and $V_2 = V\setminus V_1$.  
\end{proof}

\noindent{\bf Remarks on addition/removal}
\begin{enumerate}
\item If we {\em remove an edge} then the value of the quadratic form decreases since one of the terms on the RHS of \eqref{eq:qform} disappears. Coupled with Proposition~\ref{prp:lap-sd}(2), this tells us that removing an edge from a balanced vertex cannot make it unbalanced. 
\item If we {\em add an edge} then the value of the quadratic form increases and it is no longer obvious that 0 is an eigenvalue of the new Laplacian.
\item If we {\em remove a vertex} then the smallest eigenvalue is less than equal to the smallest eigenvalue since the eigenvalues of a principle submatrix interlace the eigenvalues of the matrix~\cite[Cor. 2.2]{haemers-LAA:1995}. This gives us a roundabout way of proving Proposition~\ref{prp:subgraphs}. Note that interlacing gives us an upper bound as well. If $\lambda_i$ are the eigenvalues of the original graph and $\lambda_i'$ of the modified graph then $\lambda_1' \leq \lambda_1 \leq \lambda_{n-1}'$. 
\\
The relation is $\lambda_1-1\leq \lambda_1'$ (see Weak Interlacing Theorem, \cite{Lotker-JLA:2007}). So, this relation will not help to prove Proposition~\ref{prp:subgraphs}.
\item If we {\em add a vertex} then again the smallest eigenvalue may increase due to the interlacing property.
\end{enumerate}

\begin{proposition}[\cite{belardo2014balancedness}]
    \label{prp:balancedness}
    Let $0 \le \lambda_1 \le \lambda_2 \le \cdots \le \lambda_n$ be the eigenvalues of the  Laplacian of $\Gamma$. Let $\nu(\Gamma), (\epsilon(\Gamma))$ denote the frustration number (and frustration index), i.e. the minimum no. of vertices (and edges) to be deleted such that the signed graph is balanced. Then, 
    
    \begin{equation*}
        \lambda_1(\Gamma) \le \nu(\Gamma) \le \epsilon(\Gamma)
    \end{equation*}
\end{proposition}

\begin{proof}
    1. $\lambda_1(\Gamma) \le \epsilon(\Gamma)$
\end{proof}

\begin{definition}
Given a function $\theta: V \rightarrow \{-1,1\}$, called a {\em switching function}, the signed graph $\Gamma^\theta=(V,\sigma^\theta)$ obtained by applying $\theta$ to $\Gamma = (V,\sigma)$ is the signed graph in which for all $(u,v) \in E$,  $\sigma^\theta(u,v) = \theta(u) \sigma(u,v) \theta(v)$. 

Two signed graphs $\Gamma_1$ and $\Gamma_2$ are are said to be {\em switching equivalent} if there is a switching function $\theta$ such that $\Gamma_2 = \Gamma_1^\theta$. We denote this by $\Gamma_1 \sim \Gamma_2$.
\end{definition}
No one has written the following explicitly, so just putting it down for our benefit. 
\begin{proposition}
Switching equivalence is an equivalence relation.
\end{proposition}
\begin{proof}
Reflexivity and transitivity are straightforward so we just argue for symmetry. This follows from the fact that for any switching function $\theta$, $(\Gamma^\theta)^\theta = \Gamma$ since $\theta(u)^2 \sigma(u,v) \theta(v)^2 = \sigma(u,v)$. This means that $\theta$ is its own inverse when it comes to switching.
\end{proof}

\begin{proposition}
\label{prp:switching-balanced}
$(G,\sigma)$ is balanced iff it is switching equivalent to $(G, +)$ where $+$ maps all edges to $+1$.
\end{proposition}
\begin{proof}
First assume $(G,\sigma)$ is balanced. If $(V_1, V_2)$ is the partition that balances $(G,\sigma)$, consider the switching function $\theta$ such that $\theta(v) = -1$ for all $v \in V_1$ and $\theta(v) = $ for all $v \in V_2$. 

If $(G,\sigma)$ is switching equivalent to $(G,+)$ let $\theta$ be a switching function that transforms one to the other. It is easy to verify that the partition $(\{v : \theta(v) = 1\}, \{v : \theta(v) = -1\})$ is a balance partition for $(G,\sigma)$.
\end{proof}

Since all acyclic signed graphs are balanced we know that for a signed graph $(G,\sigma)$ with $n$ vertices there is a $k < n$ such that the removal of $k$ vertices makes the remaining signed graph balanced. Suppose $\Sigma$ is the set of all mappings from $E$ to $\{-1,1\}$. Let $S_k$, $1 \leq k < n$, be the set of all $\sigma \in \Sigma$ such that $(G,\sigma)$ can be balanced by the removal of exactly $k$ vertices.  Then $S_0$ is the precisely the set of all mappings for which $G$ is balanced. Proposition~\ref{prp:switching-balanced} can be restated as follows: The equivalence class of the mapping $+$ under the relation $\sim$ is precisely $S_0$. 

Proposition~\ref{prp:switching-balanced} raises the following natural question: Given a graph $G$, is $S_k$ an equivalence class of $\sim$ for all values of $k$?

Zaslavsky~\cite{zaslavsky-dam:1982} observed the following property of the equivalence classes of $\sim$:
\begin{lemma}
If $\Gamma$ is a signed graph and $T$ is a maximal forest in $\Gamma$ then each switching equivalent class of sign functions has a unique representative which is $+$ on $T$. 

Moreover, given {\em any} sign function $\sigma$ on $T$ each class has a unique representative that agrees with $\sigma$ on $T$.
\end{lemma}







\subsubsection{Observations by Kartik} 
\begin{observation}
Current balance does not change on a flipping operation. In other words, $S(\Gamma^{\theta}) = S(\Gamma)$. Hence, MFN is not really a problem ?
\sm{This is true if you flip all the nodes or just a single node. What about the case when you flip a few nodes? That means the edges associated to only these few will change their signs once (flip) or twice (remains same).}

\sm{Kartik, My main concern is similar to yours. Defining a switching function on a few nodes is tricky. We are still working on it.}

\sm{The next observations seem to assume that switching function has been applied to every node --- am I missing something? }

\ks{Doesn't a switching function defined as follows flip only the nodes belonging to the set $B$ -

\[ \theta(v) = \left\{ \begin{array}{rr}
-1, & v \in B\\
+1, & \text{otherwise}
\end{array}\right.\]}

\sm{It is in MFN, but not according definition 2.1. Do your proofs assume MFN mechanism. If yes, I will go over. Just a note: we will change the switching function in MFN. Currently it lacks practical motivation. We will update this changed definition soon.}

\ks{I think they are fine according to the general definition of switching function. }

\end{observation}
Li and Li~\cite{li-tjm:2016} define
\begin{definition}
Two matrices $M_1$ and $M_2$ of order $n$ are called \textit{signature similar} if there exists a signature matrix, that is, a diagonal matrix $S = \mathrm{diag}(s_1, s_2, \cdots, s_n)$ with diagonal entries $s_i = \pm 1$ such that $M_2 = S M_1 S$.
\end{definition}
\begin{lemma} [\cite{hou2003laplacian}]
Let $\Gamma_1 = (G, \sigma_1)$ and $\Gamma_2 = (G, \sigma_2)$  be signed graphs on the same underlying graph G. Then $\Gamma_1 \sim \Gamma_2$ iff $L(\Gamma_1)$ and $L(\Gamma_2)$ are signature similar. 
\end{lemma}
This is easy to prove. Note that $\Gamma_1 \sim \Gamma_2$ means that $\Gamma_1$ is switching equivalent to $\Gamma_2$ or $\Gamma_2 = \Gamma_1^{\theta}$ for some $\theta$ (as defined earlier).

\begin{lemma}
The eigenvalues of $L(\Gamma^{\theta})$ are same as eigenvalues of $L(\Gamma)$ for all switching functions $\theta$. 
\end{lemma}

\begin{proof}
The eigenvalues of $L(\Gamma^{\theta})$ are solutions to the equation:
$\left| L(\Gamma^{\theta}) - \lambda I \right| = 0$. From previous lemma, $L(\Gamma^{\theta}) = S L(\Gamma) S$. Hence, the equation becomes $\left| S L(\Gamma) S - \lambda I \right| = 0$. Note that $SIS = I$. Thus, we get that the eigenvalues of $L(\Gamma^{\theta})$ are solutions to $\left| S (L(\Gamma) - \lambda I) S \right| = 0$. 

Since $|S|^{2} = 1$, one can simplify this equation to $\left| L(\Gamma) - \lambda I \right| = 0$, solutions of which are eigenvalues to $L(\Gamma)$.
\end{proof}

\begin{theorem}
$S(\Gamma^{\theta}) = S(\Gamma)$
\end{theorem}

\begin{proof}
Suppose $S(\Gamma^{\theta})$ is greater (i.e. has greater no. of vertices) than $S(\Gamma)$. Then, note that  $T = (S(\Gamma^{\theta}))^{\theta^{-1}}$ is a subgraph of $\Gamma$ (since inversion of switching is possible). Using the previous lemma, one can see that eigenvalues of $L(S(\Gamma^{\theta}))$ are same as that of $L(T)$. But since $S(\Gamma^{\theta})$ is balanced, its smallest eigenvalue must be $0$ and hence that of $T$. Hence $T$ is balanced. By definition, $S(\Gamma)$ must have more no. of vertices than $T$, which has same no. of vertices as $S(\Gamma^{\theta})$. Hence, we have a contradiction.
\end{proof}



